Large Neighborhood Search and Bitmask Dynamic Programming for Wireless Mobile Charging Electric Vehicle Routing Problems in Medical Transportation

The transition to electric vehicles (EVs) is critical to achieving sustainable transportation, but challenges such as limited driving range and insufficient charging infrastructure have hindered the widespread adoption of EVs, especially in time-sensitive logistics such as medical transportation. This paper presents a new model to break through this barrier by combining wireless mobile charging technology with optimization. We propose the Wireless Mobile Charging Electric Vehicle Routing Problem (WMC-EVRP), which enables Medical Transportation Electric Vehicles (MTEVs) to be charged while traveling via Mobile Charging Carts (MCTs). This eliminates the time wastage of stopping for charging and ensures uninterrupted operation of MTEVs for such time-sensitive transportation problems. However, in this problem, the decisions of these two types of heterogeneous vehicles are coupled with each other, which greatly increases the difficulty of vehicle routing optimizations. To address this complex problem, we develop a mathematical model and a tailored meta-heuristic algorithm that combines Bit Mask Dynamic Programming (BDP) and Large Neighborhood Search (LNS). The BDP approach efficiently optimizes charging strategies, while the LNS framework utilizes custom operators to optimize the MTEV routes under capacity and synchronization constraints. Our approach outperforms traditional solvers in providing solutions for medium and large instances. Using actual hospital locations in Singapore as data, we validated the practical applicability of the model through extensive experiments and provided important insights into minimizing costs and ensuring the timely delivery of healthcare services.

==> Sections/DPOriginal.tex <==
% 4 DP
% 5. Algo: ALNS+operator

\section{Bitmasking Dynamic Programming-based Operator}

In this section, we introduce a DP algorithm tailored to determine the charging edges of the EVRP. The proposed approach leverages the strengths of DP to systematically explore all feasible states, ensuring that we can identify optimal or near-optimal solutions efficiently. 

The DP algorithm takes the routes of delivery trucks as inputs, after they have been determined through LNS which will be discussed further in Algorithm \ref{Section:Algorithm}, the DP algorithm constructs solutions iterating through the potential states of the battery charge and routes. This method allows for precise calculation of feasible routes by maintaining and updating the state of the battery’s charge at each step. 

As for Bitmask DP, we have incorporated several specialized techniques:
\begin{enumerate}
    \item 
\end{enumerate}

\begin{algorithm}[htp]
\caption{Battery Charge State DP Algorithm}
\label{BatteryChargeStateDP}
\begin{algorithmic}[1]
\STATE \textbf{Input:} $f$ (required battery charge at each node), $dis$ (distance between nodes), $p$ (charge consumption rate), $Max$ (maximum battery capacity)
\STATE Initialize charge consumption $charge \leftarrow [x \times p \text{ for } x \text{ in } dis]$
\STATE Initialize DP table $dp \leftarrow \text{zeros}(2^{L+1}, \text{dtype=int})$ where $L \leftarrow \text{length}(f)$
\STATE Initialize visitation state $vis \leftarrow \text{zeros}(2^{L+1}, \text{dtype=int})$
\STATE $dp[0] \leftarrow Max$
\STATE $tot \leftarrow 0$
\STATE Initialize infinite negative value $INF \leftarrow -99999$
\FOR{$i \leftarrow 1$ to $L-1$}
    \FOR{$j \leftarrow 0$ to $(1 << (i - 1)) - 1$}
        \STATE $tot \leftarrow tot + 1$
        \STATE $k \leftarrow j | (1 << (i - 1))$
        \IF{$vis[j] == 1$}
            \STATE \textbf{continue}
        \ENDIF
        \IF{$dp[j] < 0$}
            \STATE $dp[j] \leftarrow INF$
            \STATE $vis[j] \leftarrow -1$
            \STATE $dp[k] \leftarrow INF$
            \STATE $vis[k] \leftarrow -1$
        \ENDIF
        \STATE $dp[k] \leftarrow \min(dp[j] - dis[i] + charge[i], Max)$
        \STATE $dp[j] \leftarrow dp[j] - dis[i]$
        \IF{$dp[j] \geq f[i]$}
            \STATE $vis[j] \leftarrow 1$
            \STATE \textbf{append} $j$ \textbf{to} charge\_node
        \ENDIF
        \IF{$dp[k] \geq f[i]$}
            \STATE $vis[k] \leftarrow 1$
            \STATE \textbf{append} $k$ \textbf{to} charge\_node
        \ENDIF
    \ENDFOR
\ENDFOR
\STATE \textbf{Output:} charge\_node
\end{algorithmic}
\end{algorithm}

The framework of the DP algorithm is given in 


The algorithm starts by initializing several key variables and data structures. It calculates the charge required to travel between nodes based on a given charge consumption rate. The maximum battery capacity is defined, and a dynamic programming table (\texttt{dp}) is initialized to keep track of the battery's charge state at different points along the route. Additionally, a visitation state table (\texttt{vis}) is set up to mark whether a particular state has been visited and whether it satisfies the necessary conditions.

The main part of the algorithm involves updating the DP table to reflect the possible charge states as the vehicle progresses through each node. For each node in the route (except the starting node), the algorithm considers all possible subsets of the previous nodes, represented in binary form. This allows the algorithm to explore all possible combinations of charging and traveling between nodes.

For each combination, the algorithm calculates a new state by adding the current node to the subset. It updates the battery's charge state for both the current subset and the new state, considering the distance traveled and the charge consumed or gained. If a state's charge is below zero, it is marked as invalid. Valid states are updated in the DP table, and their feasibility is checked against the required charge at the next node. If a state satisfies the requirements, it is marked as visited and added to the list of feasible charging nodes (\texttt{charge\_node}).

The algorithm's structure ensures that all possible charging strategies are explored efficiently. By using binary representation and bitwise operations, it can quickly evaluate and update the charge states for different subsets of nodes. This approach allows the algorithm to handle complex routes and charging requirements without excessive computational overhead.

The result of the algorithm is a list of feasible charging nodes, which indicates where the vehicle can charge to ensure that it has enough battery to complete the route. Therefore, the DP process output a list of synergized routes with fixed costs (with cost function given in ~\eqref{eq1}). The optimization process will then involves an exploration over the feasible synergized routes only, which will be further discussed in the next section \ref{Section:Algorithm}. 

An alternative to DP is the Naive Traversal approach for determining charging decisions. Which involves iterating through each possible arc and evaluating whether or not to charge at each node. This method evaluates all potential combinations of charging and non-charging states, resulting in a combinatorial explosion of possibilities. The time complexity for this approach is typically \(O(2^n \cdot n!)\), where \(n\) is the number of nodes. This complexity arises because the method must explore all permutations of node sequences, making it infeasible for larger instances.

In contrast, our Bitmasking DP approach offers a more efficient solution as we leverage the power of bitmask to represent states. Each state in the DP represents a particular configuration of charging decisions and remaining battery levels, allowing for the efficient reuse of previously computed results. Our approach reduces redundant calculations by storing the results of sub-problems, thus avoiding the repeated evaluation of the same state. The time complexity for the our approach is \(O(n \cdot 2^n)\). A comparison between the two algorithm complexities has been presented \ref{DPtime}. 

\begin{figure}[htbp]
\centering
\begin{minipage}{0.64\textwidth}
\includegraphics[width=1\textwidth]{pic/DPvsTraversal.jpg}
\label{DPtime}
\end{minipage}
\caption{DP and Naive Traversal Running time}
\centering
\end{figure}

The Bitmasking DP should be better suited to our MCEVRP problem setting because it effectively narrows down the search space to only those configurations that maintain feasible battery levels while minimizing energy consumption. By optimizing the charging decisions based on the current state and the available charging opportunities, the DP approach achieves a balance between computational efficiency and solution accuracy.
